How to Not Measure Disentanglement

To evaluate disentangled representations several metrics have been proposed. However, theoretical guarantees for conventional metrics of disentanglement are missing. Moreover, conventional metrics do not have a consistent correlation with the outcomes of qualitative studies. In this paper we analyze metrics of disentanglement and their properties. We conclude that existing metrics of disentanglement were created to reflect different characteristics of disentanglement and do not satisfy two basic desirable properties: (1) assign a high score to representations that are disentangled according to the definition; and (2) assign a low score to representations that are entangled according to the definition. In addition, we propose a new metric of disentanglement and prove that it satisfies both of the properties.

==> 05-experiments.tex <==
%!TEX root = ./icml2020_anna.tex

\section{Experiments}

In this section we describe our experiments.
We compare the proposed metric, \OurMeasure{}, with two conceptually similar metrics: MIG and DCI.
To this end, we consider two experimental conditions.
Due to space constraints, we only present the experimental setup and implications of the experiments; a detailed description of the results is given in Appendix~\ref{experiments}.

\subsection{Spearman rank correlation between metrics}
Following \citep{locatello2018challenging}, we explore how the metrics agree.
We provide tables with correlation scores between the metrics in Appendix~\ref{rank_correlation}.

\textbf{Results.}
Not surprisingly, we observe that \OurMeasure{} strongly correlates with MIG and DCI on the dSprites~\citep{higgins2016beta} and Cars3D~\citep{reed2015deep} datasets.
However, these datasets are artificial datasets, on which all metrics are correlated and the MIG and DCI metrics are strongly correlated.
Conceptually , \OurMeasure{} is between these two metrics, and consequently, it also strongly correlates with them on these artificial datasets.

\subsection{Different behavior of  \OurMeasure{}, MIG and DCI}
In this section we examine the difference between  \OurMeasure{} and MIG, and \OurMeasure{} and DCI. 
In particular, we show examples where \OurMeasure{} and MIG, and \OurMeasure{} and DCI, do not agree on which of the two representations is the most disentangled representation.
This experiment provides a better understanding of the differences between the metrics and what exactly the metrics penalize.
In Appendix~\ref{differences} we explain the behavior of the metrics by exploring the matrices of informativeness of representations.
Below we give the details of the experiment and its results.

\subsubsection{Comparison of \OurMeasure{} and MIG}
%
In this section, we provide an example of two representations for which \OurMeasure{} and MIG disagree over which of the two representations is the more disentangled representation, and we provide the outcomes of the comparison of the representations.
In particular, we compare two representations obtained by the $\beta$-TCVAE model~\citep{chen2018isolating} and the AnnealedVAE model~\citep{burgess2018understanding}, trained on the Cars3D dataset.
In~\citep{locatello2018challenging} they are numbered 10402 and 10587, respectively;
their matrices of informativeness are given in the Appendix, in Figures~\ref{mig_small_dcimig_large} and~\ref{mig_large_dcimig_small} correspondingly.

\textbf{Implications.} 
MIG provides high scores to compact latent representations, while \OurMeasure{} does not penalize representations in which several latent factors capture the same generative factor.
%
\subsubsection{Comparison of \OurMeasure{} and DCI}
In this section, we provide an example of two representations for which \OurMeasure{} and DCI disagree over which of the two representations is the more disentangled representation; and provide the outcomes of the comparison of the representations.
In particular, we compare the representations obtained by two models: the two $\beta$-TCVAE models trained on the Cars3D dataset; within ~\citep{locatello2018challenging} they are numbered 10429 and 10264.
Their matrices of informativeness are given in the Appendix, in Figures~\ref{mig_small_dcimig_large} and ~\ref{mig_large_dcimig_small} correspondingly.

\textbf{Implications.} 
DCI provides high scores to the latent representations in which all the latent factors are disentangled, independently of whether the latent factors capture different generative factors.
While \OurMeasure{} provides high scores to representations that contain for each generative factor at least one latent disentangle latent dimension, which reflects this factor and it is indifferent as to whether the remaining latent factors are entangled or disentangled.
